Precision Gating: Improving Neural Network Efficiency with Dynamic Dual-Precision Activations

We propose precision gating (PG), an end-to-end trainable dynamic dual-precision quantization technique for deep neural networks. PG computes most features in a low precision and only a small proportion of important features in a higher precision to preserve accuracy. The proposed approach is applicable to a variety of DNN architectures and significantly reduces the computational cost of DNN execution with almost no accuracy loss. Our experiments indicate that PG achieves excellent results on CNNs, including statically compressed mobile-friendly networks such as ShuffleNet. Compared to the state-of-the-art prediction-based quantization schemes, PG achieves the same or higher accuracy with 2.4$\times$ less compute on ImageNet. PG furthermore applies to RNNs. Compared to 8-bit uniform quantization, PG obtains a 1.2% improvement in perplexity per word with 2.7$\times$ computational cost reduction on LSTM on the Penn Tree Bank dataset. Code is available at: https://github.com/cornell-zhang/dnn-gating

==> alg/sp-backprop.tex <==
\begin{algorithm}[H]
\SetAlgoLined

\BF{Input:} $\M{I}$, $B_{lb}$\;
\BF{Parameters:} $\M{W}$, $\Delta$\;
\BF{Output:} $\M{O}$\;

\BF{Define} $\M{O}_{hb} = \mathbf{W} * (\mathbf{I}_{hb} << B_{lb})$\;
\BF{Define} $\M{O}_{lb} = \mathbf{W} * \mathbf{I}_{lb}$\;

\While{Forward}{
    $\mathbf{mask} = \mathbf{1}_{\mathbf{O}_{hb} > \Delta}$\;
    $\M{O} = \M{O}_{hb} + \M{mask}^{2} \odot \M{O}_{lb} $\;
}
\While{Backward}{
    \BF{Define} $S(\M{O}_{hb}, \Delta) = \frac{1}{1+e^{\epsilon(\M{O}_{hb}-\Delta)}} \approx \mathbf{mask}$\;
    $\frac{\partial \mathbf{O}}{\partial \mathbf{W}} = \frac{\partial \mathbf{O}_{hb}}{\partial \mathbf{W}} + \mathbf{mask}^{2} \odot \frac{\partial \mathbf{O}_{lb}}{\partial \mathbf{W}}$\;
    $\frac{\partial \mathbf{O}}{\partial \Delta}  \approx  \frac{\partial \mathbf{O}}{\partial \mathbf{mask}} \frac{\partial S(\M{O}_{hb}, \Delta)}{\partial \Delta}  = 2 \cdot \mathbf{mask} \odot \mathbf{O}_{lb} \frac{\partial S(\M{O}_{hb}, \Delta)}{\partial \Delta}$\;
    Update $\M{W}$ and $\Delta$\;
}
\caption{Feed-Forward and Back-Propagation} 
\label{alg:sp-backprop}
\end{algorithm}

==> fig-tex/fig-experiment-results.tex <==
\begin{figure}[htb]
\centering

\begin{subfigure}{0.35\textwidth}
 \centering
\includegraphics[width=0.97\linewidth]{fig-tex/fig-pdf/shiftnet-pg-results.pdf}
\caption{ShifNet-20 CIFAR-10}
\label{fig:shiftnet-cifar10-figure}
\end{subfigure}
\begin{subfigure}{0.35\textwidth}
\includegraphics[width=0.97\linewidth]{fig-tex/fig-pdf/resnet-pg-results.pdf}
\caption{ResNet-18 CIFAR-10}
\label{fig:resnet-cifar10-figure}
\end{subfigure}

\begin{subfigure}{0.35\textwidth}
\includegraphics[width=0.97\linewidth]{fig-tex/fig-pdf/shufflenet-pg-results.pdf}
\caption{ShuffleNet ImageNet}
\label{fig:shufflenet-imagenet-figure}
\end{subfigure}
\begin{subfigure}{0.35\textwidth}
\includegraphics[width=0.97\linewidth]{fig-tex/fig-pdf/lstm-pg-results.pdf}
\caption{LSTM PTB}
\label{fig:lstm-ptb-figure}
\end{subfigure}
 
\caption{\BF{Precision gating results on CNNs}}
\vspace{-15pt}
\label{fig:overall-results}
\end{figure}

==> tab/hardware-time.tex <==
\begin{table}[htb]
    \renewcommand{\arraystretch}{1.2}
    \addtolength{\tabcolsep}{0pt}
    \caption{\BF{ResNet-18 model speedup}}
    \label{tab:gpu-speedup}
    \centering
    \scalebox{1.0}{
    \begin{tabular}{cccc}
    
    \toprule

    Method & Speedup & Platform & Inference/Back-Propagation  \\
    \midrule
    PG & 1.5$\times$ & GPU & Both  \\
    \midrule
    SeerNet & 1.4$\times$ & CPU & Inference Only \\
    \bottomrule

    \end{tabular}}
\end{table}

==> tab/tab-experiment-lstm.tex <==
% \begin{table*}[tb]
% \vskip -0.1in
% \hfill
% \begin{minipage}{0.34\linewidth}
%   \centering
%   \begin{small}
%   \caption{\BF{PG on LSTM --} the dataset used is Penn Tree Bank (PTB). The metric is perplexity per word (PPW) and lower is better.}
%   \label{tab:lstm-ptb-results}
%   \vspace{3px}
%       \begin{tabular}{c@{\hskip4pt} c@{\hskip4pt} | c@{\hskip4pt}  c@{\hskip4pt}}
%         \toprule
%         \multicolumn{2}{c|}{Base} & \multicolumn{2}{c}{PG}\\
    
%         Bits & PPW   & Bits & PPW  \\
%         \midrule
%         fp   & 110.1 & & \\
%         8   & 109.8 & \textbf{3.0} & \textbf{108.5} \\
%         4   & 110.8 & \textbf{2.9} & \textbf{109.3} \\
%         3   & 112.5 & \textbf{2.5} & \textbf{111.6} \\
%         2   & 124.9 & \textbf{1.9} & \textbf{118.8} \\
%         \bottomrule
%       \end{tabular}
%   \end{small}
% \end{minipage}
% \hfill
% \begin{minipage}{0.60\linewidth}
%   \centering
%   \begin{small}
%   \caption{\BF{Precision gating vs. zero-prediction\cite{song2018prediction} --} under the same bitwidth settings $B$ and $B_{hb}$, precision gating provides better accuracy than zero-prediction.}
%   \label{tab:zero-pred}
%   \vspace{3px}
%       \begin{tabular}{c|c@{\hskip4pt} c@{\hskip4pt} c@{\hskip4pt} c@{\hskip4pt} c@{\hskip4pt}}
%         \toprule
%         & & \multicolumn{2}{c}{Zero-Pred} & \multicolumn{2}{c}{PG}   \\
%         \cmidrule(r){3-4} \cmidrule(r){5-6}
%         & $B$/$B_{hb}$ & Bits & Acc & Bits & Acc \\
%         \midrule
%       ShiftNet-20 & 5 / 3           & 4.1 & 88.6 & \textbf{4.0} & \textbf{89.1}     \\
%           CIFAR-10 & 3 / 1           & 1.5 & 82.8 & \textbf{1.4} & \textbf{83.4}    \\
%         \midrule
%       ResNet-18  & 4 / 3           & 3.5 & 91.2 & \textbf{3.4} & \textbf{91.7}    \\
%       CIFAR-10   & 3 / 2           & 2.5 & 90.9 & \textbf{2.2} & \textbf{91.2}    \\
%         \midrule
%                  & $B$/$B_{hb}$ & Bits & PPW & Bits & PPW \\
%             LSTM & 3 / 2           & 2.5 & 120.3 & \textbf{2.5} & \textbf{111.6}   \\
%              PTB & 3 / 1           & 2.0 & 330.3 & \textbf{1.9} & \textbf{118.8}   \\
%         \bottomrule
%       \end{tabular}
%   \end{small}
% \end{minipage}
% \hfill
% \vskip -0.1in
% \end{table*}


\begin{table}[htb]
    \renewcommand{\arraystretch}{1.2}
    \addtolength{\tabcolsep}{-4pt} % reduce space between columns by -2pt
    \caption{\BF{PG on LSTM --} the dataset used is Penn Tree Bank (PTB). The metric is perplexity per word (PPW) and lower is better.}
    \label{tab:lstm-ptb-results}
    % \vspace{3px}
    \centering
    \scalebox{1.0}{
    \begin{tabular}{c@{\hskip4pt} c@{\hskip4pt} | c@{\hskip4pt}  c@{\hskip4pt}}
    
        \toprule
        \multicolumn{2}{c|}{Base} & \multicolumn{2}{c}{PG}\\
    
        Bits & PPW   & Bits & PPW  \\
        \midrule
        fp   & 110.1 & & \\
        8   & 109.8 & \textbf{3.0} & \textbf{108.5} \\
        4   & 110.8 & \textbf{2.9} & \textbf{109.3} \\
        3   & 112.5 & \textbf{2.5} & \textbf{111.6} \\
        2   & 124.9 & \textbf{1.9} & \textbf{118.8} \\
        \bottomrule

    \end{tabular}}
\end{table}

==> tab/top5-acc.tex <==
\begin{table}[htb]
    \caption{\BF{Top-5 accuracy -- } the top-5 accuracy of Precision gating (PG) is reported for ResNet-18 on CIFAR-10 and ShuffleNet V2 0.5$\times$ on ImageNet. "fp" is floating-point accuracy.}
    \label{tab:top5-acc}
    % \vspace{3px}
    \renewcommand{\arraystretch}{1.2}
    \addtolength{\tabcolsep}{-2pt} % reduce space between columns by -4
    \centering
    \scalebox{0.9}{
    \begin{tabular}{c|cccc}
    
    \toprule
    & $B$/$B_{hb}$ & $B_{\text{avg}}$ & Top-1 Accu. & Top-5 Accu.\\
    \midrule
    ResNet-18   & 4/3 & 3.2 & 91.7 & 99.8 \\
    (fp top-1 91.7\%)    & 3/2 & 2.1 & 91.2 & 99.7 \\
    (fp top-5 99.8\%) & 2/1 & 1.3 & 90.6 & 99.6 \\
    \midrule
    ShuffleNet V2 0.5$\times$  & 6/4 & 4.8 & 59.7 & 81.6 \\
    (fp top-1 59.0\%) & 6/4 & 4.7 & 59.3 & 81.3 \\
    (fp top-5 81.5\%) & 5/3 & 4.1 & 58.0 & 80.3 \\
    \bottomrule
    
    \end{tabular}}
\end{table}
